Tracking and Reconstructing Hand Object Interactions from Point Cloud Sequences in the Wild

In this work, we tackle the challenging task of jointly tracking hand object pose and reconstructing their shapes from depth point cloud sequences in the wild, given the initial poses at frame 0. We for the first time propose a point cloud based hand joint tracking network, HandTrackNet, to estimate the inter-frame hand joint motion. Our HandTrackNet proposes a novel hand pose canonicalization module to ease the tracking task, yielding accurate and robust hand joint tracking. Our pipeline then reconstructs the full hand via converting the predicted hand joints into a template-based parametric hand model MANO. For object tracking, we devise a simple yet effective module that estimates the object SDF from the first frame and performs optimization-based tracking. Finally, a joint optimization step is adopted to perform joint hand and object reasoning, which alleviates the occlusion-induced ambiguity and further refines the hand pose. During training, the whole pipeline only sees purely synthetic data, which are synthesized with sufficient variations and by depth simulation for the ease of generalization. The whole pipeline is pertinent to the generalization gaps and thus directly transferable to real in-the-wild data. We evaluate our method on two real hand object interaction datasets, e.g. HO3D and DexYCB, without any finetuning. Our experiments demonstrate that the proposed method significantly outperforms the previous state-of-the-art depth-based hand and object pose estimation and tracking methods, running at a frame rate of 9 FPS.

==> tex/03_problem.tex <==
\vspace{-3mm}
\section{Problem Formulation}
\vspace{-5mm}
\label{sec:prob_form}
\paragraph{Notations} In this paper, we deploy the following notations: %superscripts $(\cdot)^h$ and $(\cdot)^o$ denote variables associated with the hand and the object, respectively; 
right subscripts $(\cdot)_t$ represent quantities at the time step $t$; and left $_{C}(\cdot)$, $_{H}(\cdot)$, $_{O}(\cdot)$ denote variables in camera space, canonical hand space (with zero global translation and identity rotation) and canonical object spaces, respectively. 

\vspace{-3mm}
\paragraph{Problem setting} Given a live stream of segmented hand and object point clouds$\{_C\PC^{hand}, _C\PC^{obj}\}_t$, along with initial hand joint positions $\J_{init}$ and initial object pose $\{\R_{init}^{obj}, \T_{init}^{obj}\}$ at frame $0$, we aim to recover canonical object shape $_O\M^{obj}$ and its pose $\{\R_{t}^{obj}, \T_{t}^{obj}\}$ along with hand joint positions $\J_t$ and hand reconstruction, including hand shape $_H\M_t^{hand} =MANO(\boldsymbol{\theta}_t, \boldsymbol{\beta})$ ($\boldsymbol{\theta}_t$ and $\boldsymbol{\beta}$ are pose and shape code  of MANO hand, respectively) and global hand pose $\{\R_{t}^{hand}, \T_{t}^{hand}\}$, for all the following frames $t$ in an online manner. 



==> tex/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
%The checklist follows the references.  Please
%read the checklist guidelines carefully for information on how to answer these
%questions.  For each question, change the default \answerTODO{} to \answerYes{},
%\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
%justification to your answer}, either by referencing the appropriate section of
%your paper or providing a brief inline description.  For example:
%\begin{itemize}
%  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%  \item Did you include the license to the code and datasets? \answerNA{}
%\end{itemize}
%Please do not modify the questions and only use the provided macros for your
%answers.  Note that the Checklist section does not count towards the page
%limit.  In your paper, please delete this instructions block and only keep the
%Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{} We discuss the limitations, which is also our future work, in conclusion \ref{conclusion}.
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{} We will release the data and the code upon acceptance.
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{} We discuss it in chapter \ref{train detail} as well as in our supplementary materials.
    \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}  
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{} We report it in supplementary materials.
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{} We will mention it in our code repository.
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{} We will release the URL in our code repository.
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{} We checked the licenses of the datasets we used and satisfies their requirements.
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{} Our proposed dataset only contains common objects which carries no personally identifiable information nor offensive content.
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
